Ridge partial correlation screening for ultrahigh-dimensional data

Variable selection in ultrahigh-dimensional linear regression is challenging due to its high computational cost. Therefore, a screening step is usually conducted before variable selection to significantly reduce the dimension. Here we propose a novel and simple screening method based on ordering the absolute sample ridge partial correlations. The proposed method takes into account not only the ridge regularized estimates of the regression coefficients but also the ridge regularized partial variances of the predictor variables providing sure screening property without strong assumptions on the marginal correlations. Simulation study and a real data analysis show that the proposed method has a competitive performance compared with the existing screening procedures. A publicly available software implementing the proposed screening accompanies the article.

==> C-computation.tex <==
\section{Fast statistical computation }
\label{sec:comfw}

In this section we describe how ridge partial correlation is computed
in practice. From Definition \ref{def:rpc}, recall that $R_{i,\lambda}$ is defined in terms of the quantities
$v_{iy, \lambda}, v_{i, \lambda}$ and $ v_{y, \lambda}$. %  and as
% \[R_{i,\lambda} = -v_{iy, \lambda}/\{v_{i, \lambda}\times v_{y,
%   \lambda}\}^{1/2}.\]
We now illustrate the computation of  $v_{iy, \lambda}, v_{i, \lambda},$ and $ v_{y, \lambda}$ separately. By the Woodbury matrix identity we have
\begin{equation}\label{comp:xxt}
(X^\top X + \lambda I)^{-1} = \dfrac{1}{\lambda}I-\dfrac{1}{\lambda}X^{\top}(XX^{\top}+\lambda I)^{-1}X.
\end{equation}

Note that  \[v_{y, \lambda} = (\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}X(X^{\top}X+\lambda I)^{-1}X^{\top}\tilde{Y})^{-1}.\]
Let $W = XX^{\top} + \lambda I$. Thus using \eqref{comp:xxt}, we have
\begin{equation}
\begin{split}
\label{comp:vy}
    v_{y, \lambda} &= (\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}X(X^{\top}X+\lambda I)^{-1}X^{\top}\tilde{Y})^{-1}\\
                   &= \Bigg(\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}X\left\{\dfrac{1}{\lambda}I-\dfrac{1}{\lambda}X^{\top}(XX^{\top}+\lambda I)^{-1}X\right\}X^{\top}\tilde{Y}\Bigg)^{-1} \\
                   &= \Big(\tilde{Y}^{\top}\tilde{Y} - \dfrac{1}{\lambda}\tilde{Y}^{\top}XX^{\top}\tilde{Y} + \dfrac{1}{\lambda}\tilde{Y}^{\top}XX^{\top}(XX^{\top}+\lambda I)^{-1}XX^{\top}\tilde{Y}\Big)^{-1}\\
                   &= \Big(\tilde{Y}^{\top}\tilde{Y} - \dfrac{1}{\lambda}\tilde{Y}^{\top}XX^{\top}\tilde{Y} + \dfrac{1}{\lambda}\tilde{Y}^{\top}XX^{\top}\tilde{Y} - \tilde{Y}^{\top}(XX^{\top}+\lambda I)^{-1}XX^{\top}\tilde{Y}\Big)^{-1}\\
                   &= (\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}\tilde{Y} + \lambda \tilde{Y}^{\top}(XX^{\top}+\lambda I)^{-1}\tilde{Y})^{-1}\\
                   &= \dfrac{1}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}}
\end{split}                   
\end{equation}

Similarly, by Definition \ref{def:rpc} and \eqref{comp:xxt}, we have
\begin{equation} 
\label{comp:viy}
    \begin{split}
       v_{iy, \lambda} &= \left\{ -(X^{\top}X + \lambda I)^{-1}X^{\top}\tilde{Y} (\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}X(X^{\top}X+\lambda I)^{-1}X^{\top}\tilde{Y})^{-1} \right\}_i\\
                       &= \left\{-\dfrac{\left[\dfrac{1}{\lambda}I-\dfrac{1}{\lambda}X^{\top}(XX^{\top}+\lambda I)^{-1}X\right]X^{\top}\tilde{Y}}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}}\right\}_i\\
                       &= \left\{-\dfrac{\dfrac{1}{\lambda}\left[X^{\top}\tilde{Y}-X^{\top}\tilde{Y}+\lambda X^{\top}(XX^{\top}+\lambda I)^{-1}\tilde{Y}\right]}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}}\right\}_i\\
                       &= -\dfrac{X^{\top}_iW^{-1}\tilde{Y}}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}}
    \end{split}
\end{equation}

Lastly, by Definition \ref{def:rpc}, \eqref{comp:xxt}, \eqref{comp:viy}, 
we have
\begin{equation}
\label{comp:vi}
    \begin{split}
        v_{i, \lambda} &= \left\{(X^{\top}X + \lambda I)^{-1}\right\}_{ii} + \frac{\left\{(X^{\top}X + \lambda I)^{-1}X^{\top}\tilde{Y}\tilde{Y}^{\top}X (X^{\top}X + \lambda I)^{-1}\right\}_{ii}}{\tilde{Y}^{\top}\tilde{Y} - \tilde{Y}^{\top}X(X^{\top}X+\lambda I)^{-1}X^{\top}\tilde{Y}}\\
                       &= \left\{\dfrac{1}{\lambda}I-\dfrac{1}{\lambda}X^{\top}(XX^{\top}+\lambda I)^{-1}X\right\}_{ii} + \dfrac{(X^{\top}_iW^{-1}\tilde{Y})^2}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}}\\
                       &= \dfrac{1}{\lambda} + \dfrac{(X^{\top}_iW^{-1}\tilde{Y})^2}{\lambda \tilde{Y}^{\top}W^{-1}\tilde{Y}} - \dfrac{1}{\lambda}X^{\top}_iW^{-1}X_i
    \end{split}
\end{equation}

\subsection{Algorithm for computing ridge partial correlations}
We can further accelerate the computation of ridge partial correlations by using Cholesky decomposition. Let $S$ be the Cholesky factor of $W$ such that $S$ is the upper triangular matrix satisfying $W = S^{\top}S$. Let $\theta = S^{-\top}\tilde{Y}, u_i = S^{-\top}X_i$. Then $\tilde{Y}^{\top}W^{-1}\tilde{Y} = \theta^{\top}\theta, X^{\top}_iW^{-1}\tilde{Y} = u^{\top}_i\theta$ and $X^{\top}_iW^{-1}X_i = u^{\top}_iu_i$. Substitute these equations into \eqref{comp:vy}, \eqref{comp:viy} and \eqref{comp:vi}, we get the following algorithm for efficiently computing the ridge partial correlations:
\begin{enumerate}
    \item Given $X, \tilde{Y}$ and $\lambda$, compute $W = XX^{\top} + \lambda I$.
    \item Compute the Cholesky factor of $W$, denoted by $S$, which is the upper triangular matrix satisfying $W = S^{\top}S$.
    \item Compute $\theta = S^{-\top}\tilde{Y}$ and $v_{y, \lambda} = 1/(\lambda \theta^{\top}\theta).$
    \item For each $i = 1,2,\ldots,p$, 
    \begin{itemize}
     \item[--] compute $u_i = S^{-\top}X_i$, $v_{iy, \lambda} = -v_{y,\lambda}\cdot u_i^{\top}\theta$ and 
     $v_{i, \lambda} = \lambda^{-1} + v_{y, \lambda}(u_i^{\top}\theta)^2 - \lambda^{-1}u^{\top}_iu_i.$
     \item[--] Compute $R_{i,\lambda} = -v_{iy, \lambda}/\{v_{i, \lambda}\times v_{y, \lambda}\}^{1/2}$
    \end{itemize}
\end{enumerate}

In the above algorithm, the last step can be paralleled over
$i$ as implemented in the R package {\it rpc} \citep{r:rpc}. Overall, the computational complexity of the above algorithm is
$O(n^3) + O(n^2p)$ where the $O(n^3)$ term correspond to computing the
Cholesky factorization of $XX^\top + \lambda I$ and the $O(n^2p)$ term
arises due to computing $XX^\top$ and for computing $u_i$'s. Thus,
encouragingly, the computational complexity of the proposed method of
implementing the RPC screening is the same as that of the HOLP.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sim-table-exp1.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} 
% &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.456 & 0    & 0.107 & 0 & 0.823 & 0.44 & 0.772 & 0.18 & 0.093 & 0 & 0.671 & 0.02 & 0.414 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.002 & 0 & 0.026 & 0    & 0.026 & 0    & 0     & 0 & 0     & 0    & 0.017 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2}
% &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$  
                              & 0.456 & 0    & 0.107 & 0 & 0.823 & 0.44 & 0.772 & 0.18 & 0.093 & 0 & 0.672 & 0.02 & 0.414 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.002 & 0 & 0.026 & 0    & 0.026 & 0    & 0     & 0 & 0     & 0    & 0.017 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC3}  
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.456 & 0    & 0.107 & 0 & 0.822 & 0.44 & 0.772 & 0.18 & 0.093 & 0 & 0.669 & 0.02 & 0.413 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.002 & 0 & 0.026 & 0    & 0.026 & 0    & 0     & 0 & 0     & 0    & 0.017 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC(ALL)} 
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$  
                              & 0.456 & 0    & 0.107 & 0 & 0.823 & 0.44 & 0.772 & 0.18 & 0.094 & 0 & 0.674 & 0.02 & 0.414 & 0    \\
                              %\hline
%\multicolumn{1}{l}{BITS1}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
 %                             $n$                    & 0.311 & 0.01 & 0.092 & 0 & 0.787 & 0.49 & 0.58  & 0.02 & 0.097 & 0 & 0.092 & 0    & 0.454 & 0    \\
                              %PP                   & 0.121 & 0    & 0.014 & 0 & 0.194 & 0    & 0.218 & 0    & 0.001 & 0 & 0.032 & 0    & 0.069 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.001 & 0 & 0.032 & 0    & 0.028 & 0    & 0.001 & 0 & 0     & 0    & 0.021 & 0    \\
                              %\hline
% \multicolumn{1}{l}{BITS2}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.352 & 0    & 0.1   & 0 & 0.793 & 0.51 & 0.621 & 0.03 & 0.102 & 0 & 0.177 & 0    & 0.456 & 0    \\
%                               PP                   & 0.128 & 0    & 0.014 & 0 & 0.203 & 0    & 0.22  & 0    & 0.001 & 0 & 0.03  & 0    & 0.073 & 0    \\
%                               EBIC                 & 0.001 & 0    & 0.001 & 0 & 0.032 & 0    & 0.028 & 0    & 0.001 & 0 & 0     & 0    & 0.021 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.176 & 0    & 0.066 & 0 & 0.588 & 0.18 & 0.302 & 0    & 0.07  & 0 & 0.023 & 0    & 0.364 & 0    \\
%                               PP                   & 0.038 & 0    & 0.001 & 0 & 0.133 & 0    & 0.121 & 0    & 0.001 & 0 & 0.003 & 0    & 0.044 & 0    \\
%                               EBIC                 & 0.001 & 0    & 0.001 & 0 & 0.032 & 0    & 0.028 & 0    & 0.001 & 0 & 0     & 0    & 0.021 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)}
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$ 
                               & 0.483 & 0.01 & 0.18  & 0 & 0.867 & 0.66 & 0.733 & 0.12 & 0.172 & 0 & 0.188 & 0    & 0.581 & 0.01 \\
                              %PP                   & 0.156 & 0    & 0.018 & 0 & 0.217 & 0    & 0.257 & 0    & 0.001 & 0 & 0.04  & 0    & 0.083 & 0    \\\hline
\multicolumn{1}{l}{HOLP} 
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$    
                             & 0.457 & 0    & 0.107 & 0 & 0.823 & 0.44 & 0.772 & 0.18 & 0.094 & 0 & 0.61  & 0    & 0.416 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.002 & 0 & 0.026 & 0    & 0.026 & 0    & 0     & 0 & 0.001 & 0    & 0.017 & 0    \\\hline
\multicolumn{1}{l}{FR} 
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$ 
                              & 0.151 & 0    & 0.063 & 0 & 0.224 & 0    & 0.23  & 0    & 0.069 & 0 & 0.087 & 0    & 0.089 & 0    \\
                              %EBIC                 & 0.001 & 0    & 0.001 & 0 & 0.032 & 0    & 0.028 & 0    & 0.001 & 0 & 0     & 0    & 0.021 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                             & 0.47  & 0    & 0.174 & 0 & 0.888 & 0.6  & 0.828 & 0.25 & 0.176 & 0 & 0.013 & 0    & 0.51  & 0   \\\hline
\end{tabular}


==> sim-table-exp2.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1}
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.736 & 0.02 & 0.172 & 0 & 0.987 & 0.94 & 0.968 & 0.77 & 0.159 & 0 & 0.826 & 0.17 & 0.536 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.098 & 0    & 0.117 & 0    & 0     & 0 & 0.013 & 0    & 0.033 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2} 
%&                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.737 & 0.02 & 0.171 & 0 & 0.987 & 0.94 & 0.968 & 0.77 & 0.159 & 0 & 0.823 & 0.17 & 0.536 & 0    \\
                               %EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.098 & 0    & 0.118 & 0    & 0     & 0 & 0.013 & 0    & 0.033 & 0    \\
                               %\hline
\multicolumn{1}{l}{RPC3}  %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.737 & 0.02 & 0.172 & 0 & 0.987 & 0.94 & 0.967 & 0.76 & 0.159 & 0 & 0.826 & 0.18 & 0.535 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.098 & 0    & 0.117 & 0    & 0     & 0 & 0.013 & 0    & 0.033 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC(ALL)} %                          &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                   
                              & 0.738 & 0.02 & 0.172 & 0 & 0.987 & 0.94 & 0.968 & 0.77 & 0.159 & 0 & 0.828 & 0.18 & 0.536 & 0    \\%\hline
% \multicolumn{1}{l}{BITS1}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.544 & 0    & 0.128 & 0 & 0.976 & 0.92 & 0.847 & 0.23 & 0.178 & 0 & 0.204 & 0    & 0.56  & 0.01 \\
%                               PP                   & 0.308 & 0    & 0.036 & 0 & 0.347 & 0    & 0.346 & 0    & 0.006 & 0 & 0.089 & 0    & 0.126 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.006 & 0 & 0.177 & 0    & 0.137 & 0    & 0.003 & 0 & 0     & 0    & 0.046 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.641 & 0    & 0.148 & 0 & 0.996 & 0.98 & 0.884 & 0.39 & 0.177 & 0 & 0.342 & 0.02 & 0.577 & 0    \\
%                               PP                   & 0.324 & 0    & 0.027 & 0 & 0.352 & 0    & 0.358 & 0    & 0.008 & 0 & 0.113 & 0    & 0.124 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.006 & 0 & 0.177 & 0    & 0.137 & 0    & 0.003 & 0 & 0     & 0    & 0.046 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.323 & 0    & 0.093 & 0 & 0.923 & 0.8  & 0.477 & 0    & 0.094 & 0 & 0.05  & 0    & 0.497 & 0    \\
%                               PP                   & 0.153 & 0    & 0.011 & 0 & 0.291 & 0    & 0.236 & 0    & 0.003 & 0 & 0.016 & 0    & 0.084 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.006 & 0 & 0.177 & 0    & 0.137 & 0    & 0.003 & 0 & 0     & 0    & 0.046 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                         &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.729 & 0.04 & 0.244 & 0 & 1     & 1    & 0.928 & 0.53 & 0.254 & 0 & 0.354 & 0.02 & 0.667 & 0.02 \\
                             % PP                   & 0.36  & 0    & 0.042 & 0 & 0.387 & 0    & 0.399 & 0    & 0.008 & 0 & 0.116 & 0    & 0.147 & 0    \\
                             %\hline
\multicolumn{1}{l}{HOLP}  %                             &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.737 & 0.02 & 0.17  & 0 & 0.987 & 0.94 & 0.967 & 0.76 & 0.166 & 0 & 0.761 & 0.07 & 0.538 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.098 & 0    & 0.118 & 0    & 0     & 0 & 0.016 & 0    & 0.033 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}  %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$                    
                             & 0.31  & 0    & 0.077 & 0 & 0.34  & 0    & 0.339 & 0    & 0.088 & 0 & 0.127 & 0    & 0.133 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.006 & 0 & 0.177 & 0    & 0.137 & 0    & 0.003 & 0 & 0     & 0    & 0.046 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                   & 0.758 & 0.04 & 0.24  & 0 & 0.996 & 0.98 & 0.978 & 0.85 & 0.204 & 0 & 0.003 & 0    & 0.604 & 0.02\\\hline
\end{tabular}

==> sim-table-exp3.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1}  %                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.903 & 0.33 & 0.236 & 0 & 0.999 & 0.99 & 0.99  & 0.92 & 0.201 & 0 & 0.927 & 0.54 & 0.645 & 0.01 \\
                              %EBIC                 & 0.084 & 0    & 0.013 & 0 & 0.143 & 0    & 0.169 & 0    & 0     & 0 & 0.07  & 0    & 0.04  & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2}%                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.903 & 0.33 & 0.237 & 0 & 0.999 & 0.99 & 0.99  & 0.92 & 0.202 & 0 & 0.927 & 0.54 & 0.645 & 0.01 \\
                               %EBIC                 & 0.084 & 0    & 0.013 & 0 & 0.143 & 0    & 0.169 & 0    & 0     & 0 & 0.07  & 0    & 0.04  & 0    \\
                               %\hline
\multicolumn{1}{l}{RPC3}  %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.903 & 0.33 & 0.236 & 0 & 0.999 & 0.99 & 0.99  & 0.92 & 0.201 & 0 & 0.927 & 0.54 & 0.645 & 0.01 \\
                               %EBIC                 & 0.084 & 0    & 0.013 & 0 & 0.143 & 0    & 0.17  & 0    & 0     & 0 & 0.07  & 0    & 0.04  & 0    \\
                               %\hline
\multicolumn{1}{l}{RPC(ALL)}  %                          &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$                    
                               & 0.903 & 0.33 & 0.237 & 0 & 0.999 & 0.99 & 0.99  & 0.92 & 0.202 & 0 & 0.927 & 0.54 & 0.645 & 0.01 \\%\hline
% \multicolumn{1}{l}{BITS1}                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.791 & 0.14 & 0.188 & 0 & 1     & 1    & 0.938 & 0.55 & 0.206 & 0 & 0.488 & 0.04 & 0.671 & 0.01 \\
%                               PP                   & 0.592 & 0.05 & 0.051 & 0 & 0.416 & 0    & 0.446 & 0    & 0.011 & 0 & 0.3   & 0.01 & 0.164 & 0    \\
%                               EBIC                 & 0.092 & 0    & 0.011 & 0 & 0.316 & 0    & 0.218 & 0    & 0.004 & 0 & 0     & 0    & 0.078 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.828 & 0.24 & 0.203 & 0 & 1     & 1    & 0.954 & 0.68 & 0.219 & 0 & 0.65  & 0.11 & 0.678 & 0    \\
%                               PP                   & 0.614 & 0.05 & 0.042 & 0 & 0.433 & 0    & 0.469 & 0    & 0.013 & 0 & 0.34  & 0.03 & 0.174 & 0    \\
%                               EBIC                 & 0.092 & 0    & 0.011 & 0 & 0.316 & 0    & 0.217 & 0    & 0.004 & 0 & 0     & 0    & 0.078 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.592 & 0.05 & 0.11  & 0 & 1     & 1    & 0.592 & 0    & 0.113 & 0 & 0.097 & 0    & 0.596 & 0.01 \\
%                               PP                   & 0.442 & 0.01 & 0.016 & 0 & 0.332 & 0    & 0.336 & 0    & 0.006 & 0 & 0.041 & 0    & 0.112 & 0    \\
%                               EBIC                 & 0.092 & 0    & 0.011 & 0 & 0.316 & 0    & 0.218 & 0    & 0.004 & 0 & 0     & 0    & 0.078 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                          &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$ 
                              & 0.9   & 0.39 & 0.309 & 0 & 1     & 1    & 0.976 & 0.78 & 0.302 & 0 & 0.656 & 0.11 & 0.74  & 0.04 \\
                             % PP                   & 0.642 & 0.06 & 0.059 & 0 & 0.474 & 0    & 0.506 & 0    & 0.013 & 0 & 0.356 & 0.04 & 0.197 & 0    \\
                             %\hline
\multicolumn{1}{l}{HOLP}%                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$       
                              & 0.903 & 0.33 & 0.237 & 0 & 0.999 & 0.99 & 0.99  & 0.92 & 0.204 & 0 & 0.899 & 0.38 & 0.645 & 0.01 \\
                              %EBIC                 & 0.084 & 0    & 0.012 & 0 & 0.143 & 0    & 0.169 & 0    & 0     & 0 & 0.073 & 0    & 0.04  & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}   %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$                    
                             & 0.593 & 0.05 & 0.086 & 0 & 0.369 & 0    & 0.43  & 0    & 0.099 & 0 & 0.218 & 0    & 0.166 & 0    \\
                              %EBIC                 & 0.092 & 0    & 0.011 & 0 & 0.316 & 0    & 0.218 & 0    & 0.006 & 0 & 0     & 0    & 0.078 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                            & 0.914 & 0.39 & 0.348 & 0 & 1     & 1    & 0.997 & 0.97 & 0.238 & 0 & 0     & 0    & 0.688 & 0.02\\\hline
\end{tabular}


==> sim-table-exp4.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                         &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$    
                              & 0.969 & 0.77 & 0.318 & 0 & 1     & 1 & 0.998 & 0.98 & 0.271 & 0 & 0.968 & 0.74 & 0.67  & 0.01 \\
                              %EBIC                 & 0.184 & 0    & 0.02  & 0 & 0.26  & 0 & 0.254 & 0    & 0.003 & 0 & 0.237 & 0    & 0.048 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2} %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                  
                              & 0.969 & 0.77 & 0.316 & 0 & 1     & 1 & 0.998 & 0.98 & 0.272 & 0 & 0.968 & 0.74 & 0.67  & 0.01 \\
                              %EBIC                 & 0.184 & 0    & 0.02  & 0 & 0.261 & 0 & 0.254 & 0    & 0.003 & 0 & 0.237 & 0    & 0.048 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC3} %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.969 & 0.77 & 0.319 & 0 & 1     & 1 & 0.998 & 0.98 & 0.272 & 0 & 0.967 & 0.73 & 0.669 & 0.01 \\
                              %EBIC                 & 0.184 & 0    & 0.02  & 0 & 0.26  & 0 & 0.254 & 0    & 0.003 & 0 & 0.236 & 0    & 0.048 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC(ALL)} %                           &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                    
                              & 0.969 & 0.77 & 0.319 & 0 & 1     & 1 & 0.998 & 0.98 & 0.274 & 0 & 0.969 & 0.75 & 0.67  & 0.01 \\%\hline
% \multicolumn{1}{l}{BITS1}                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.931 & 0.58 & 0.26  & 0 & 1     & 1 & 0.981 & 0.83 & 0.284 & 0 & 0.744 & 0.29 & 0.718 & 0.01 \\
%                               PP                   & 0.829 & 0.33 & 0.072 & 0 & 0.486 & 0 & 0.56  & 0    & 0.019 & 0 & 0.527 & 0.21 & 0.199 & 0    \\
%                               EBIC                 & 0.212 & 0    & 0.022 & 0 & 0.333 & 0 & 0.301 & 0    & 0.008 & 0 & 0.002 & 0    & 0.1   & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.944 & 0.6  & 0.276 & 0 & 1     & 1 & 0.987 & 0.88 & 0.303 & 0 & 0.886 & 0.5  & 0.722 & 0.02 \\
%                               PP                   & 0.844 & 0.39 & 0.074 & 0 & 0.567 & 0 & 0.596 & 0    & 0.022 & 0 & 0.578 & 0.19 & 0.218 & 0    \\
%                               EBIC                 & 0.212 & 0    & 0.022 & 0 & 0.333 & 0 & 0.299 & 0    & 0.008 & 0 & 0.002 & 0    & 0.1   & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.831 & 0.34 & 0.114 & 0 & 1     & 1 & 0.712 & 0.07 & 0.132 & 0 & 0.2   & 0    & 0.652 & 0.01 \\
%                               PP                   & 0.717 & 0.18 & 0.026 & 0 & 0.333 & 0 & 0.416 & 0    & 0.008 & 0 & 0.073 & 0    & 0.122 & 0    \\
%                               EBIC                 & 0.209 & 0    & 0.022 & 0 & 0.333 & 0 & 0.301 & 0    & 0.007 & 0 & 0.002 & 0    & 0.1   & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                          &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                   
                              & 0.971 & 0.76 & 0.381 & 0 & 1     & 1 & 0.993 & 0.94 & 0.386 & 0 & 0.89  & 0.51 & 0.789 & 0.07 \\
                              %PP                   & 0.86  & 0.41 & 0.094 & 0 & 0.62  & 0 & 0.636 & 0.01 & 0.027 & 0 & 0.616 & 0.26 & 0.25  & 0    \\
                              %\hline
\multicolumn{1}{l}{HOLP} %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$     
                               & 0.969 & 0.77 & 0.319 & 0 & 1     & 1 & 0.998 & 0.98 & 0.276 & 0 & 0.95  & 0.59 & 0.67  & 0.01 \\
                              %EBIC                 & 0.184 & 0    & 0.02  & 0 & 0.263 & 0 & 0.254 & 0    & 0.003 & 0 & 0.241 & 0    & 0.048 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}   %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                   
                              & 0.82  & 0.33 & 0.114 & 0 & 0.366 & 0 & 0.519 & 0    & 0.1   & 0 & 0.389 & 0.03 & 0.168 & 0    \\
                              %EBIC                 & 0.209 & 0    & 0.021 & 0 & 0.333 & 0 & 0.301 & 0    & 0.007 & 0 & 0.002 & 0    & 0.1   & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                             & 0.964 & 0.71 & 0.417 & 0 & 1     & 1 & 1     & 1    & 0.221 & 0 & 0     & 0    & 0.71  & 0.05\\\hline
\end{tabular}


==> sim-table-norm1.tex <==

\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$                   
                              & 0.434                & 0                    & 0.099                & 0                    & 0.822                & 0.46                 & 0.754                & 0.18                 & 0.121                & 0                    & 0.662                & 0.03                 & 0.388                & 0                    \\
                              % EBIC                 & 0.002                & 0                    & 0.003                & 0                    & 0.014                & 0                    & 0.024                & 0                    & 0                    & 0                    & 0.001                & 0                    & 0.009                & 0                    \\
                               %\hline
\multicolumn{1}{l}{RPC2}  %                      &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$  
                               & 0.436                & 0                    & 0.099                & 0                    & 0.823                & 0.46                 & 0.756                & 0.18                 & 0.121                & 0                    & 0.664                & 0.03                 & 0.389                & 0                    \\
                               %EBIC                 & 0.002                & 0                    & 0.003                & 0                    & 0.014                & 0                    & 0.024                & 0                    & 0                    & 0                    & 0.001                & 0                    & 0.009                & 0                    \\
                               %\hline
\multicolumn{1}{l}{RPC3}  %                      &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$ 
                               & 0.434                & 0                    & 0.099                & 0                    & 0.822                & 0.46                 & 0.753                & 0.18                 & 0.121                & 0                    & 0.666                & 0.03                 & 0.387                & 0                    \\
                               %EBIC                 & 0.002                & 0                    & 0.003                & 0                    & 0.014                & 0                    & 0.024                & 0                    & 0                    & 0                    & 0.001                & 0                    & 0.009                & 0                    \\
                               %\hline
\multicolumn{1}{l}{RPC(ALL)}  %                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$ 
                               & 0.436                & 0                    & 0.099                & 0                    & 0.823                & 0.46                 & 0.756                & 0.18                 & 0.122                & 0                    & 0.67                 & 0.03                 & 0.389                & 0                    \\%\hline
% \multicolumn{1}{l}{BITS1}                       &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.292                & 0                    & 0.082                & 0                    & 0.794                & 0.47                 & 0.551                & 0.01                 & 0.127                & 0                    & 0.088                & 0                    & 0.439                & 0                    \\
%                               PP                   & 0.131                & 0                    & 0.023                & 0                    & 0.19                 & 0                    & 0.189                & 0                    & 0.016                & 0                    & 0.029                & 0                    & 0.069                & 0                    \\
%                               EBIC                 & 0.002                & 0                    & 0.002                & 0                    & 0.021                & 0                    & 0.026                & 0                    & 0.015                & 0                    & 0                    & 0                    & 0.012                & 0                    \\\hline
% \multicolumn{1}{l}{BITS2}                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.333                & 0                    & 0.086                & 0                    & 0.777                & 0.45                 & 0.577                & 0.01                 & 0.134                & 0                    & 0.153                & 0                    & 0.428                & 0                    \\
%                               PP                   & 0.118                & 0                    & 0.021                & 0                    & 0.206                & 0                    & 0.189                & 0                    & 0.017                & 0                    & 0.034                & 0                    & 0.065                & 0                    \\
%                               EBIC                 & 0.002                & 0                    & 0.002                & 0                    & 0.021                & 0                    & 0.026                & 0                    & 0.015                & 0                    & 0                    & 0                    & 0.012                & 0                    \\\hline
% \multicolumn{1}{l}{BITS3}                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.179                & 0                    & 0.072                & 0                    & 0.646                & 0.28                 & 0.288                & 0                    & 0.074                & 0                    & 0.027                & 0                    & 0.367                & 0                    \\
%                               PP                   & 0.037                & 0                    & 0.003                & 0                    & 0.126                & 0                    & 0.116                & 0                    & 0.016                & 0                    & 0.006                & 0                    & 0.039                & 0                    \\
%                               EBIC                 & 0.002                & 0                    & 0.002                & 0                    & 0.021                & 0                    & 0.026                & 0                    & 0.015                & 0                    & 0                    & 0                    & 0.012                & 0                    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$
                               & 0.456                & 0                    & 0.173                & 0                    & 0.878                & 0.64                 & 0.694                & 0.05                 & 0.201                & 0                    & 0.163                & 0                    & 0.553                & 0.01                 \\
                               %PP                   & 0.156                & 0                    & 0.031                & 0                    & 0.223                & 0                    & 0.22                 & 0                    & 0.017                & 0                    & 0.038                & 0                    & 0.079                & 0                    \\
                               %\hline
\multicolumn{1}{l}{HOLP} %                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              % $n$
                              & 0.434                & 0                    & 0.099                & 0                    & 0.824                & 0.47                 & 0.753                & 0.18                 & 0.121                & 0                    & 0.592                & 0.01                 & 0.391                & 0                    \\
                              % EBIC                 & 0.002                & 0                    & 0.003                & 0                    & 0.014                & 0                    & 0.024                & 0                    & 0                    & 0                    & 0.001                & 0                    & 0.009                & 0                    \\
                              %\hline
\multicolumn{1}{l}{FR}   %                        &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$ 
                               & 0.154                & 0                    & 0.062                & 0                    & 0.209                & 0                    & 0.21                 & 0                    & 0.079                & 0                    & 0.091                & 0                    & 0.093                & 0                    \\
                              % EBIC                 & 0.002                & 0                    & 0.002                & 0                    & 0.021                & 0                    & 0.026                & 0                    & 0.015                & 0                    & 0                    & 0                    & 0.012                & 0                    \\
                              %\hline
\multicolumn{1}{l}{SIS}                                                & 0.462                & 0                    & 0.142                & 0                    & 0.884                & 0.63                 & 0.832                & 0.29                 & 0.2                  & 0                    & 0.019                & 0                    & 0.483                & 0                   \\\hline
\end{tabular}


==> sim-table-norm3.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                           &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.893 & 0.33 & 0.238 & 0 & 1     & 1 & 0.998 & 0.98 & 0.183 & 0 & 0.923 & 0.46 & 0.634 & 0.02 \\
                              %EBIC                 & 0.043 & 0    & 0.004 & 0 & 0.16  & 0 & 0.159 & 0    & 0.002 & 0 & 0.037 & 0    & 0.042 & 0    \\
                             % \hline
\multicolumn{1}{l}{RPC2}   %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              % $n$                    &       &      &       &   &       &   &       &      &       &   &       &      &       &      \\
                              %EBIC                
                              & 0.893 & 0.33 & 0.238 & 0 & 1     & 1 & 0.998 & 0.98 & 0.184 & 0 & 0.922 & 0.45 & 0.635 & 0.02 \\
                              %\hline
\multicolumn{1}{l}{RPC3} %                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$  
                              & 0.893 & 0.33 & 0.238 & 0 & 1     & 1 & 0.998 & 0.98 & 0.182 & 0 & 0.923 & 0.46 & 0.634 & 0.02 \\
                             
                             % EBIC                 & 0.043 & 0    & 0.004 & 0 & 0.159 & 0 & 0.16  & 0    & 0.002 & 0 & 0.037 & 0    & 0.042 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC(ALL)} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.893 & 0.33 & 0.238 & 0 & 1     & 1 & 0.998 & 0.98 & 0.184 & 0 & 0.924 & 0.47 & 0.635 & 0.02 \\%\hline
% \multicolumn{1}{l}{BITS1}  %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               %$n$
%                               & 0.786 & 0.08 & 0.183 & 0 & 1     & 1 & 0.944 & 0.62 & 0.193 & 0 & 0.427 & 0.01 & 0.674 & 0.02 \\
%                               %PP                  & 0.579 & 0.01 & 0.044 & 0 & 0.409 & 0 & 0.451 & 0    & 0.009 & 0 & 0.231 & 0.01 & 0.164 & 0    \\
%                               EBIC                 & 0.048 & 0    & 0.01  & 0 & 0.321 & 0 & 0.22  & 0    & 0.001 & 0 & 0     & 0    & 0.084 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.828 & 0.1  & 0.201 & 0 & 1     & 1 & 0.966 & 0.76 & 0.214 & 0 & 0.613 & 0.06 & 0.67  & 0.02 \\
%                               PP                  & 0.607 & 0    & 0.054 & 0 & 0.439 & 0 & 0.478 & 0    & 0.009 & 0 & 0.261 & 0.01 & 0.172 & 0    \\
%                               EBIC                 & 0.048 & 0    & 0.01  & 0 & 0.321 & 0 & 0.221 & 0    & 0.001 & 0 & 0     & 0    & 0.084 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.594 & 0.01 & 0.098 & 0 & 1     & 1 & 0.58  & 0    & 0.102 & 0 & 0.09  & 0    & 0.617 & 0.03 \\
%                               PP                  & 0.389 & 0    & 0.012 & 0 & 0.332 & 0 & 0.339 & 0    & 0.003 & 0 & 0.032 & 0    & 0.118 & 0    \\
%                               EBIC                 & 0.048 & 0    & 0.01  & 0 & 0.321 & 0 & 0.219 & 0    & 0.001 & 0 & 0     & 0    & 0.084 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)}%                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.897 & 0.35 & 0.29  & 0 & 1     & 1 & 0.98  & 0.85 & 0.289 & 0 & 0.621 & 0.06 & 0.74  & 0.06 \\
                              %PP                   & 0.639 & 0.01 & 0.068 & 0 & 0.48  & 0 & 0.511 & 0    & 0.012 & 0 & 0.281 & 0.01 & 0.198 & 0    \\
                             % \hline
\multicolumn{1}{l}{HOLP}  %                                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.893 & 0.33 & 0.239 & 0 & 1     & 1 & 0.998 & 0.98 & 0.181 & 0 & 0.899 & 0.37 & 0.636 & 0.02 \\
                              %EBIC                 & 0.043 & 0    & 0.004 & 0 & 0.16  & 0 & 0.16  & 0    & 0.002 & 0 & 0.048 & 0    & 0.042 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}    %                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.573 & 0    & 0.096 & 0 & 0.368 & 0 & 0.416 & 0    & 0.082 & 0 & 0.194 & 0    & 0.16  & 0    \\
                              %EBIC                 & 0.048 & 0    & 0.01  & 0 & 0.321 & 0 & 0.219 & 0    & 0.001 & 0 & 0     & 0    & 0.084 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                                                & 0.901 & 0.39 & 0.349 & 0 & 1     & 1 & 0.999 & 0.99 & 0.209 & 0 & 0.001 & 0    & 0.675 & 0.02\\\hline
\end{tabular}


==> sim-table-norm4.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.96  & 0.69 & 0.324 & 0 & 1     & 1 & 0.999 & 0.99 & 0.36  & 0    & 0.974 & 0.8  & 0.69  & 0.01 \\
                              %EBIC                 & 0.152 & 0    & 0.02  & 0 & 0.251 & 0 & 0.262 & 0    & 0.006 & 0    & 0.199 & 0    & 0.046 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2} %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$ 
                              & 0.96  & 0.69 & 0.324 & 0 & 1     & 1 & 0.999 & 0.99 & 0.362 & 0    & 0.976 & 0.81 & 0.69  & 0.01 \\
                              %EBIC                 & 0.152 & 0    & 0.02  & 0 & 0.251 & 0 & 0.262 & 0    & 0.006 & 0    & 0.198 & 0    & 0.046 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC3}  %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.96  & 0.69 & 0.323 & 0 & 1     & 1 & 0.999 & 0.99 & 0.36  & 0    & 0.973 & 0.79 & 0.69  & 0.01 \\
                              %EBIC                 & 0.152 & 0    & 0.02  & 0 & 0.25  & 0 & 0.261 & 0    & 0.006 & 0    & 0.199 & 0    & 0.046 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC(ALL)} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$    
                             & 0.96  & 0.69 & 0.326 & 0 & 1     & 1 & 0.999 & 0.99 & 0.362 & 0    & 0.976 & 0.81 & 0.69  & 0.01 \\%\hline
% \multicolumn{1}{l}{BITS1} %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    &       &      &       &   &       &   &       &      &       &      &       &      &       &      \\
%                               PP                  & 0.857 & 0.31 & 0.079 & 0 & 0.473 & 0 & 0.55  & 0    & 0.021 & 0    & 0.556 & 0.19 & 0.208 & 0    \\
%                               EBIC                 & 0.168 & 0    & 0.02  & 0 & 0.333 & 0 & 0.296 & 0    & 0.009 & 0    & 0.001 & 0    & 0.104 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    &       &      &       &   &       &   &       &      &       &      &       &      &       &      \\
%                               PP                   & 0.862 & 0.35 & 0.07  & 0 & 0.536 & 0 & 0.587 & 0    & 0.023 & 0    & 0.596 & 0.2  & 0.221 & 0    \\
%                               EBIC                 & 0.167 & 0    & 0.02  & 0 & 0.333 & 0 & 0.297 & 0    & 0.009 & 0    & 0.001 & 0    & 0.104 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    &       &      &       &   &       &   &       &      &       &      &       &      &       &      \\
%                               PP                   & 0.709 & 0.12 & 0.032 & 0 & 0.333 & 0 & 0.411 & 0    & 0.01  & 0    & 0.098 & 0.01 & 0.13  & 0    \\
%                               EBIC                 & 0.168 & 0    & 0.02  & 0 & 0.333 & 0 & 0.296 & 0    & 0.009 & 0    & 0.001 & 0    & 0.104 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.968 & 0.75 & 0.357 & 0 & 1     & 1 & 0.996 & 0.96 & 0.453 & 0.02 & 0.898 & 0.57 & 0.787 & 0.07 \\
                             % PP                  & 0.889 & 0.42 & 0.094 & 0 & 0.598 & 0 & 0.638 & 0.02 & 0.028 & 0    & 0.618 & 0.24 & 0.258 & 0    \\
                             %\hline
\multicolumn{1}{l}{HOLP}%                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                               %$n$
                               & 0.96  & 0.69 & 0.324 & 0 & 1     & 1 & 0.999 & 0.99 & 0.364 & 0    & 0.956 & 0.67 & 0.691 & 0.01 \\
                              %EBIC                 & 0.152 & 0    & 0.02  & 0 & 0.25  & 0 & 0.261 & 0    & 0.006 & 0    & 0.2   & 0    & 0.046 & 0    \\
                             % \hline
\multicolumn{1}{l}{FR} %                                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.828 & 0.3  & 0.117 & 0 & 0.358 & 0 & 0.506 & 0    & 0.136 & 0    & 0.386 & 0.04 & 0.174 & 0    \\
                              %EBIC                 & 0.168 & 0    & 0.019 & 0 & 0.333 & 0 & 0.296 & 0    & 0.009 & 0    & 0.001 & 0    & 0.104 & 0    \\
                             % \hline
                              
\multicolumn{1}{l}{SIS}                                                 & 0.964 & 0.71 & 0.417 & 0 & 1     & 1 & 1     & 1    & 0.202 & 0    & 0     & 0    & 0.728 & 0.03\\\hline
\end{tabular}


==> sim-table-t1.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$    
                              & 0.436 & 0 & 0.106 & 0 & 0.806 & 0.4  & 0.787 & 0.19 & 0.107 & 0 & 0.671 & 0.02 & 0.411 & 0    \\
                              
                              %EBIC                 & 0     & 0 & 0     & 0 & 0.023 & 0    & 0.023 & 0    & 0     & 0 & 0.001 & 0    & 0.012 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC2}    %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.436 & 0 & 0.106 & 0 & 0.806 & 0.4  & 0.787 & 0.19 & 0.107 & 0 & 0.672 & 0.02 & 0.411 & 0    \\
                             % EBIC                 & 0     & 0 & 0     & 0 & 0.023 & 0    & 0.023 & 0    & 0     & 0 & 0.001 & 0    & 0.012 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC3}  %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.436 & 0 & 0.104 & 0 & 0.804 & 0.4  & 0.786 & 0.19 & 0.107 & 0 & 0.67  & 0.02 & 0.411 & 0    \\
                              % EBIC                 & 0     & 0 & 0     & 0 & 0.023 & 0    & 0.023 & 0    & 0     & 0 & 0.001 & 0    & 0.012 & 0    \\
                             % \hline
\multicolumn{1}{l}{RPC(ALL)} %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.436 & 0 & 0.106 & 0 & 0.806 & 0.4  & 0.787 & 0.19 & 0.108 & 0 & 0.673 & 0.02 & 0.411 & 0    \\%\hline
% \multicolumn{1}{l}{BITS1}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.304 & 0 & 0.073 & 0 & 0.744 & 0.41 & 0.572 & 0.01 & 0.107 & 0 & 0.096 & 0    & 0.44  & 0.02 \\
%                               PP                   & 0.133 & 0 & 0.011 & 0 & 0.193 & 0    & 0.204 & 0    & 0.006 & 0 & 0.033 & 0    & 0.074 & 0    \\
%                               EBIC                 & 0     & 0 & 0     & 0 & 0.031 & 0    & 0.027 & 0    & 0.002 & 0 & 0.001 & 0    & 0.013 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.351 & 0 & 0.094 & 0 & 0.824 & 0.5  & 0.617 & 0.02 & 0.114 & 0 & 0.16  & 0    & 0.454 & 0.01 \\
%                               PP                  & 0.123 & 0 & 0.012 & 0 & 0.196 & 0    & 0.208 & 0    & 0.004 & 0 & 0.042 & 0    & 0.075 & 0    \\
%                               EBIC                 & 0     & 0 & 0     & 0 & 0.031 & 0    & 0.027 & 0    & 0.002 & 0 & 0.001 & 0    & 0.013 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.168 & 0 & 0.072 & 0 & 0.594 & 0.21 & 0.292 & 0    & 0.07  & 0 & 0.032 & 0    & 0.361 & 0    \\
%                               PP                  & 0.036 & 0 & 0.001 & 0 & 0.121 & 0    & 0.12  & 0    & 0.002 & 0 & 0.008 & 0    & 0.046 & 0    \\
%                               EBIC                 & 0     & 0 & 0     & 0 & 0.031 & 0    & 0.027 & 0    & 0.002 & 0 & 0.001 & 0    & 0.013 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)}%                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.461 & 0 & 0.178 & 0 & 0.873 & 0.62 & 0.719 & 0.07 & 0.178 & 0 & 0.168 & 0    & 0.572 & 0.02 \\
                              %PP                   & 0.161 & 0 & 0.016 & 0 & 0.217 & 0    & 0.234 & 0    & 0.006 & 0 & 0.047 & 0    & 0.087 & 0    \\
                              %\hline
\multicolumn{1}{l}{HOLP}%                                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.436 & 0 & 0.106 & 0 & 0.809 & 0.42 & 0.786 & 0.19 & 0.109 & 0 & 0.594 & 0    & 0.412 & 0    \\
                              %EBIC                 & 0     & 0 & 0     & 0 & 0.023 & 0    & 0.023 & 0    & 0     & 0 & 0.002 & 0    & 0.012 & 0    \\
                             % \hline
\multicolumn{1}{l}{FR} %                                    &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.162 & 0 & 0.063 & 0 & 0.219 & 0    & 0.227 & 0    & 0.071 & 0 & 0.089 & 0    & 0.09  & 0    \\
                              %EBIC                 & 0     & 0 & 0     & 0 & 0.031 & 0    & 0.027 & 0    & 0.002 & 0 & 0.001 & 0    & 0.013 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                     & 0.456 & 0 & 0.161 & 0 & 0.877 & 0.68 & 0.826 & 0.26 & 0.19  & 0 & 0.042 & 0    & 0.503 & 0.01\\\hline
\end{tabular}


==> sim-table-t2.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.743 & 0.06 & 0.177 & 0 & 0.991 & 0.96 & 0.961 & 0.7  & 0.142 & 0 & 0.823 & 0.2  & 0.544 & 0    \\
                             % EBIC                 & 0.024 & 0    & 0.007 & 0 & 0.098 & 0    & 0.109 & 0    & 0.001 & 0 & 0.016 & 0    & 0.036 & 0    \\
                            % \hline
\multicolumn{1}{l}{RPC2} %                               &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.743 & 0.06 & 0.177 & 0 & 0.991 & 0.96 & 0.961 & 0.7  & 0.147 & 0 & 0.824 & 0.2  & 0.545 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.007 & 0 & 0.098 & 0    & 0.109 & 0    & 0.001 & 0 & 0.016 & 0    & 0.036 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC3}  %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                            % $n$
                            & 0.743 & 0.06 & 0.177 & 0 & 0.991 & 0.96 & 0.961 & 0.7  & 0.141 & 0 & 0.823 & 0.2  & 0.544 & 0    \\
                             % EBIC                 & 0.024 & 0    & 0.007 & 0 & 0.098 & 0    & 0.109 & 0    & 0.001 & 0 & 0.016 & 0    & 0.036 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC(ALL)}   %                          &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$ 
                             & 0.743 & 0.06 & 0.177 & 0 & 0.991 & 0.96 & 0.961 & 0.7  & 0.148 & 0 & 0.826 & 0.2  & 0.545 & 0    \\%\hline
% \multicolumn{1}{l}{BITS1}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.601 & 0.01 & 0.138 & 0 & 0.991 & 0.97 & 0.851 & 0.29 & 0.134 & 0 & 0.26  & 0    & 0.584 & 0    \\
%                               PP                   & 0.353 & 0    & 0.031 & 0 & 0.352 & 0    & 0.352 & 0    & 0.001 & 0 & 0.13  & 0    & 0.118 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.172 & 0    & 0.131 & 0    & 0.001 & 0 & 0     & 0    & 0.049 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.661 & 0.04 & 0.152 & 0 & 0.988 & 0.95 & 0.88  & 0.28 & 0.148 & 0 & 0.406 & 0.01 & 0.584 & 0    \\
%                               PP                   & 0.346 & 0    & 0.038 & 0 & 0.35  & 0    & 0.363 & 0    & 0.001 & 0 & 0.142 & 0    & 0.122 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.172 & 0    & 0.131 & 0    & 0.001 & 0 & 0     & 0    & 0.049 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.363 & 0    & 0.084 & 0 & 0.95  & 0.85 & 0.461 & 0.01 & 0.083 & 0 & 0.057 & 0    & 0.526 & 0    \\
%                               PP                   & 0.169 & 0    & 0.009 & 0 & 0.308 & 0    & 0.236 & 0    & 0.001 & 0 & 0.02  & 0    & 0.086 & 0    \\
%                               EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.172 & 0    & 0.131 & 0    & 0.001 & 0 & 0     & 0    & 0.049 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                           &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$ 
                              & 0.751 & 0.06 & 0.243 & 0 & 0.999 & 0.99 & 0.923 & 0.45 & 0.223 & 0 & 0.418 & 0.01 & 0.688 & 0.01 \\
                              %PP                   & 0.389 & 0    & 0.047 & 0 & 0.384 & 0    & 0.399 & 0    & 0.001 & 0 & 0.159 & 0    & 0.141 & 0    \\
                              %\hline
\multicolumn{1}{l}{HOLP}   %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.743 & 0.06 & 0.177 & 0 & 0.991 & 0.96 & 0.961 & 0.7  & 0.144 & 0 & 0.782 & 0.08 & 0.545 & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.007 & 0 & 0.099 & 0    & 0.109 & 0    & 0.001 & 0 & 0.02  & 0    & 0.036 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR} %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.347 & 0    & 0.08  & 0 & 0.341 & 0    & 0.331 & 0    & 0.079 & 0 & 0.128 & 0    & 0.13  & 0    \\
                              %EBIC                 & 0.024 & 0    & 0.004 & 0 & 0.172 & 0    & 0.131 & 0    & 0.001 & 0 & 0     & 0    & 0.049 & 0    \\
                              %\hline
\multicolumn{1}{l}{SIS}                             & 0.763 & 0.08 & 0.249 & 0 & 0.996 & 0.97 & 0.982 & 0.84 & 0.209 & 0 & 0.003 & 0    & 0.614 & 0  \\\hline 
\end{tabular}


==> sim-table-t3.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1} %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.888 & 0.3  & 0.227 & 0 & 1     & 1    & 0.988 & 0.89 & 0.237 & 0 & 0.912 & 0.44 & 0.632 & 0.01 \\
                             % EBIC                 & 0.054 & 0    & 0.009 & 0 & 0.15  & 0    & 0.173 & 0    & 0.001 & 0 & 0.054 & 0    & 0.043 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC2} %                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.888 & 0.3  & 0.227 & 0 & 1     & 1    & 0.988 & 0.89 & 0.238 & 0 & 0.911 & 0.45 & 0.632 & 0.01 \\
                             % EBIC                 & 0.056 & 0    & 0.009 & 0 & 0.15  & 0    & 0.173 & 0    & 0.001 & 0 & 0.054 & 0    & 0.043 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC3}  %                                &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.888 & 0.3  & 0.227 & 0 & 1     & 1    & 0.988 & 0.89 & 0.237 & 0 & 0.913 & 0.45 & 0.632 & 0.01 \\
                             % EBIC                 & 0.053 & 0    & 0.009 & 0 & 0.15  & 0    & 0.173 & 0    & 0.001 & 0 & 0.054 & 0    & 0.043 & 0    \\
                             %\hline
\multicolumn{1}{l}{RPC(ALL)}  %                            &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.888 & 0.3  & 0.227 & 0 & 1     & 1    & 0.988 & 0.89 & 0.238 & 0 & 0.916 & 0.47 & 0.632 & 0.01 \\
                              %\hline
% \multicolumn{1}{l}{BITS1}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.779 & 0.13 & 0.171 & 0 & 1     & 1    & 0.941 & 0.61 & 0.232 & 0 & 0.449 & 0.01 & 0.677 & 0.02 \\
%                               PP                   & 0.591 & 0.03 & 0.039 & 0 & 0.402 & 0    & 0.44  & 0    & 0.009 & 0 & 0.223 & 0    & 0.17  & 0    \\
%                               EBIC                 & 0.059 & 0    & 0.011 & 0 & 0.312 & 0    & 0.223 & 0    & 0.003 & 0 & 0     & 0    & 0.084 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.839 & 0.21 & 0.188 & 0 & 1     & 1    & 0.963 & 0.72 & 0.236 & 0 & 0.613 & 0.05 & 0.673 & 0.02 \\
%                               PP                   & 0.592 & 0.03 & 0.04  & 0 & 0.434 & 0    & 0.466 & 0    & 0.01  & 0 & 0.262 & 0    & 0.177 & 0    \\
%                               EBIC                 & 0.059 & 0    & 0.01  & 0 & 0.312 & 0    & 0.222 & 0    & 0.003 & 0 & 0     & 0    & 0.084 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.589 & 0.01 & 0.088 & 0 & 0.997 & 0.99 & 0.586 & 0.02 & 0.11  & 0 & 0.072 & 0    & 0.622 & 0    \\
%                               PP                   & 0.394 & 0    & 0.016 & 0 & 0.332 & 0    & 0.339 & 0    & 0.004 & 0 & 0.031 & 0    & 0.118 & 0    \\
%                               EBIC                 & 0.059 & 0    & 0.011 & 0 & 0.311 & 0    & 0.223 & 0    & 0.003 & 0 & 0     & 0    & 0.084 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)} %                             &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.892 & 0.35 & 0.284 & 0 & 1     & 1    & 0.981 & 0.85 & 0.316 & 0 & 0.626 & 0.05 & 0.748 & 0.05 \\
                            %  PP                   & 0.642 & 0.05 & 0.054 & 0 & 0.473 & 0    & 0.504 & 0    & 0.012 & 0 & 0.277 & 0    & 0.208 & 0    \\
                            %\hline
\multicolumn{1}{l}{HOLP} %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.888 & 0.3  & 0.227 & 0 & 1     & 1    & 0.988 & 0.89 & 0.24  & 0 & 0.888 & 0.35 & 0.632 & 0.01 \\
                              %EBIC                 & 0.053 & 0    & 0.009 & 0 & 0.15  & 0    & 0.173 & 0    & 0.002 & 0 & 0.057 & 0    & 0.043 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}%                                     &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                            %  $n$
                            & 0.573 & 0.03 & 0.076 & 0 & 0.363 & 0    & 0.429 & 0    & 0.103 & 0 & 0.179 & 0    & 0.158 & 0    \\
                             % EBIC                 & 0.059 & 0    & 0.011 & 0 & 0.311 & 0    & 0.223 & 0    & 0.003 & 0 & 0     & 0    & 0.084 & 0    \\
                             %\hline
\multicolumn{1}{l}{SIS}                            & 0.892 & 0.33 & 0.308 & 0 & 1     & 1    & 0.989 & 0.9  & 0.188 & 0 & 0     & 0    & 0.684 & 0.03\\%\hline
\end{tabular}


==> sim-table-t4.tex <==
\begin{tabular}{rrr|rr|rr|rr|rr|rr|rr}
\hline\hline\multicolumn{1}{c}{Method}    & \multicolumn{12}{c}{Correlation Structure}\\

\hline%\multicolumn{1}{l}{}                        & \multicolumn{12}{c}{Theoretical $R^2 = 0.7$}                                                                                                                                                         \\
                        & \multicolumn{2}{c|}{IID}      & \multicolumn{2}{c|}{Compound} & \multicolumn{2}{c|}{Group}    & \multicolumn{2}{c|}{AR}       & \multicolumn{2}{c|}{Factor}  & \multicolumn{2}{c|}{ExtrmCor}  &
                        \multicolumn{2}{c}{SparseFactor}\\
                           & TPR            & CP         & TPR           & CP          & TPR            & CP         & TPR            & CP         & TPR           & CP         & TPR           & CP    &TPR      &CP      \\\hline
\multicolumn{1}{l}{RPC1}%                             &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                            %  $n$  
                            & 0.956 & 0.65 & 0.352 & 0 & 1     & 1 & 1     & 1    & 0.293 & 0    & 0.968 & 0.74 & 0.629 & 0.02 \\
                              %EBIC                 & 0.171 & 0    & 0.028 & 0 & 0.231 & 0 & 0.252 & 0    & 0.008 & 0    & 0.192 & 0.01 & 0.042 & 0    \\
                             % \hline
\multicolumn{1}{l}{RPC2}  %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.956 & 0.65 & 0.353 & 0 & 1     & 1 & 1     & 1    & 0.291 & 0    & 0.968 & 0.74 & 0.63  & 0.02 \\
                              %EBIC                 & 0.172 & 0    & 0.028 & 0 & 0.231 & 0 & 0.252 & 0    & 0.008 & 0    & 0.192 & 0.01 & 0.042 & 0    \\
                             % \hline
\multicolumn{1}{l}{RPC3}  %                                 &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.956 & 0.65 & 0.352 & 0 & 1     & 1 & 1     & 1    & 0.289 & 0    & 0.969 & 0.75 & 0.629 & 0.02 \\
                              %EBIC                 & 0.171 & 0    & 0.028 & 0 & 0.233 & 0 & 0.253 & 0    & 0.008 & 0    & 0.193 & 0.01 & 0.042 & 0    \\
                              %\hline
\multicolumn{1}{l}{RPC(ALL)} %                              &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.956 & 0.65 & 0.354 & 0 & 1     & 1 & 1     & 1    & 0.294 & 0    & 0.969 & 0.75 & 0.63  & 0.02 \\%\hline
% \multicolumn{1}{l}{BITS1}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.91  & 0.45 & 0.268 & 0 & 1     & 1 & 0.984 & 0.86 & 0.273 & 0    & 0.726 & 0.31 & 0.671 & 0.03 \\
%                               PP                   & 0.836 & 0.33 & 0.086 & 0 & 0.483 & 0 & 0.562 & 0    & 0.014 & 0    & 0.527 & 0.16 & 0.19  & 0    \\
%                               EBIC                 & 0.176 & 0    & 0.027 & 0 & 0.333 & 0 & 0.296 & 0    & 0.006 & 0    & 0.001 & 0    & 0.097 & 0    \\\hline
% \multicolumn{1}{l}{BITS2}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.937 & 0.56 & 0.283 & 0 & 1     & 1 & 0.996 & 0.96 & 0.297 & 0    & 0.878 & 0.51 & 0.678 & 0.01 \\
%                               PP                   & 0.854 & 0.37 & 0.086 & 0 & 0.551 & 0 & 0.602 & 0    & 0.018 & 0    & 0.597 & 0.2  & 0.203 & 0    \\
%                               EBIC                 & 0.176 & 0    & 0.027 & 0 & 0.333 & 0 & 0.297 & 0    & 0.007 & 0    & 0.001 & 0    & 0.097 & 0    \\\hline
% \multicolumn{1}{l}{BITS3}                                  &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
%                               $n$                    & 0.834 & 0.33 & 0.13  & 0 & 1     & 1 & 0.703 & 0.04 & 0.147 & 0    & 0.209 & 0.01 & 0.612 & 0.01 \\
%                               PP                   & 0.72  & 0.15 & 0.037 & 0 & 0.334 & 0 & 0.421 & 0    & 0.008 & 0    & 0.086 & 0    & 0.119 & 0    \\
%                               EBIC                 & 0.176 & 0    & 0.027 & 0 & 0.333 & 0 & 0.296 & 0    & 0.006 & 0    & 0.001 & 0    & 0.097 & 0    \\\hline
\multicolumn{1}{l}{BITS(ALL)}  %                           &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                             % $n$
                             & 0.956 & 0.68 & 0.389 & 0 & 1     & 1 & 0.998 & 0.98 & 0.378 & 0.01 & 0.882 & 0.52 & 0.741 & 0.05 \\
                              %PP                   & 0.864 & 0.38 & 0.107 & 0 & 0.609 & 0 & 0.646 & 0    & 0.022 & 0    & 0.61  & 0.21 & 0.238 & 0    \\
                              %\hline
\multicolumn{1}{l}{HOLP}%                                   &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.956 & 0.65 & 0.351 & 0 & 1     & 1 & 1     & 1    & 0.297 & 0    & 0.947 & 0.61 & 0.632 & 0.02 \\
                              %EBIC                 & 0.171 & 0    & 0.028 & 0 & 0.233 & 0 & 0.251 & 0    & 0.009 & 0    & 0.196 & 0.01 & 0.042 & 0    \\
                              %\hline
\multicolumn{1}{l}{FR}%                                    &                &             &               &              &                &             &                &             &               &             &               &       &      &       \\
                              %$n$
                              & 0.831 & 0.33 & 0.127 & 0 & 0.374 & 0 & 0.511 & 0    & 0.129 & 0    & 0.37  & 0.04 & 0.164 & 0    \\
                              %EBIC                 & 0.176 & 0    & 0.027 & 0 & 0.333 & 0 & 0.296 & 0    & 0.006 & 0    & 0.001 & 0    & 0.097 & 0    \\
                             % \hline
\multicolumn{1}{l}{SIS}                            & 0.956 & 0.65 & 0.411 & 0 & 1     & 1 & 1     & 1    & 0.221 & 0    & 0     & 0    & 0.661 & 0.04\\\hline
\end{tabular}

